Hierarchical Action Recognition: A Contrastive Video-Language Approach with Hierarchical Interactions

Video recognition remains an open challenge, requiring the identification of diverse content categories within videos. Mainstream approaches often perform flat classification, overlooking the intrinsic hierarchical structure relating categories. To address this, we formalize the novel task of hierarchical video recognition, and propose a video-language learning framework tailored for hierarchical recognition. Specifically, our framework encodes dependencies between hierarchical category levels, and applies a top-down constraint to filter recognition predictions. We further construct a new fine-grained dataset based on medical assessments for rehabilitation of stroke patients, serving as a challenging benchmark for hierarchical recognition. Through extensive experiments, we demonstrate the efficacy of our approach for hierarchical recognition, significantly outperforming conventional methods, especially for fine-grained subcategories. The proposed framework paves the way for hierarchical modeling in video understanding tasks, moving beyond flat categorization.

==> sec/0_abstract.tex <==
\begin{abstract}
% Many excellent video language learning models have been proposed for video recognition. However, these studies mainly identify all categories simultaneously through the idea of flat recognition/classification, ignoring the underlying hierarchical structure between categories. To this end, in this paper, we define the hierarchical video recognition problem and propose a video language learning framework with hierarchical interactions to perform level-by-level content recognition for hierarchically labeled videos. Moreover, to better conduct research on this hierarchical video recognition task, we specifically construct a new dataset with fine-grained annotations, developed on medical rehabilitation assessment of stroke patients. In the process of constructing the hierarchical video recognition model, we pay special attention to the interactions between category levels and use hierarchical dependencies to perform joint learning between levels. In particular, we additionally consider the affiliation of hierarchical labels and establish a top-down constraint rule to filter the recognition results at each level. Extensive experimental results demonstrate the effectiveness and explanatory power of our proposed approach.
% Video recognition is a challenging task that requires identifying various categories of content in videos. Existing methods often perform flat recognition/classification, which ignores the hierarchical structure of categories. To this end, in this paper, we define the hierarchical video recognition problem and propose a novel video-language learning framework for this, which leverages hierarchical interactions to achieve level-by-level category recognition. Specifically, our framework exploits the dependencies between category levels and uses a top-down constraint rule to filter the recognition results. We also construct a new dataset with fine-grained annotations for medical rehabilitation assessment of stroke patients, which serves as a benchmark for this task. We demonstrate the effectiveness of our framework through extensive experiments. Compared with existing methods, we can not only conduct hierarchical video recognition, but also achieve a more significant performance improvement in the recognition of more challenging subcategories.
Video recognition remains an open challenge in computer vision, requiring the identification of diverse content categories within videos.
Mainstream approaches often perform flat classification, overlooking the intrinsic hierarchical structure relating categories. 
To address this, we formalize the novel task of hierarchical video recognition, and propose a video-language learning framework tailored for hierarchical recognition. 
Specifically, our framework encodes semantic dependencies between nodes in the category hierarchy through a structured loss, and applies a top-down constraint to filter recognition predictions. We further construct a new fine-grained dataset based on medical assessments for rehabilitation of stroke patients, serving as a challenging benchmark for hierarchical recognition. 
Through extensive experiments, we demonstrate the efficacy of our approach for hierarchical recognition, significantly outperforming conventional flat classification baselines, especially for fine-grained subcategories. 
The proposed framework provides a simple yet effective approach to incorporate hierarchical modeling into video understanding tasks, paving the way for hierarchical reasoning beyond flat video categorization.
\end{abstract}

==> tab/FMA.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t]
\centering
\caption{Examples of the content and structure for the Fugl-Meyer Assessment (FMA) categories.}
\resizebox{0.90\linewidth}{!}{%
\begin{tabular}{|ll|}
\hline
\multicolumn{2}{|c|}{\textbf{Fugl-Meyer Assessment}}                                                                                                                                                                                                                         \\ \hline
\multicolumn{1}{|l|}{\textbf{Items}}                                                                                                                                                                        & \textbf{Scores}                                                \\ \hline
\multicolumn{1}{|l|}{\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}I1: Shoulder Flexion to 180\textdegree \;Test: \\ \quad\; shoulder flexes from 90\textdegree\;to 180\textdegree, elbow stays at 0\textdegree \\ \quad\; and forearm does not pronate or supinate.\end{tabular}}} & S0: Shoulder abduction or elbow flexion happens immediately when shoulder flexion starts.              \\ \cline{2-2} 
\multicolumn{1}{|l|}{}                                                                                                                                                                                      & S1: Shoulder abduction or elbow flexion happens during movement.        \\ \cline{2-2} 
\multicolumn{1}{|l|}{}                                                                                                                                                                                      & S2: Shoulder can flex to 180\textdegree, no shoulder abduction or elbow flexion. \\ \hline
\end{tabular}%
}
\label{tab:FMA}
\end{table*}
